Restoration algorithms and system performance evaluation for active imagers

This paper deals with two fields related to active imaging system. First, we begin to explore image processing algorithms to restore the artefacts like speckle, scintillation and image dancing caused by atmospheric turbulence. Next, we examine how to evaluate the performance of this kind of systems. To do this task, we propose a modified version of the german TRM3 metric which permits to get MTF-like measures. We use the database acquired during NATO-TG40 field trials to make our tests.

==> warping.tex <==
\setlength{\unitlength}{0.00087489in}
%
\begingroup\makeatletter\ifx\SetFigFontNFSS\undefined%
\gdef\SetFigFontNFSS#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
{\renewcommand{\dashlinestretch}{90}
\begin{picture}(8349,2739)(0,-10)
\put(1352,1352){\circle*{170}}
\put(5525,865){\circle{170}}
\put(6424,912){\circle{170}}
\put(6381,1733){\circle{170}}
\put(5469,1712){\circle{170}}
\put(5873,1244){\circle*{170}}
\put(913,917){\circle{170}}
\put(1819,911){\circle{170}}
\put(910,1817){\circle{170}}
\put(1813,1810){\circle{170}}
\drawline(12,2712)(3612,2712)(3612,12)
	(12,12)(12,2712)
\drawline(462,2712)(462,12)
\drawline(912,2712)(912,12)
\drawline(1362,2712)(1362,12)
\drawline(1812,2712)(1812,12)
\drawline(2262,2712)(2262,12)
\drawline(2712,2712)(2712,12)
\drawline(3162,2712)(3162,12)
\drawline(12,2262)(3612,2262)
\drawline(12,1812)(3612,1812)
\drawline(12,1362)(3612,1362)
\drawline(12,912)(3612,912)
\drawline(12,462)(3612,462)
\drawline(4737,2712)(8337,2712)(8337,12)
	(4737,12)(4737,2712)
\drawline(5187,2712)(5187,2710)(5186,2706)
	(5185,2698)(5184,2686)(5182,2668)
	(5180,2645)(5177,2618)(5173,2585)
	(5169,2547)(5165,2506)(5160,2462)
	(5156,2415)(5151,2368)(5146,2319)
	(5142,2271)(5137,2224)(5133,2177)
	(5129,2131)(5126,2087)(5123,2044)
	(5120,2003)(5117,1962)(5115,1923)
	(5113,1885)(5111,1847)(5110,1810)
	(5109,1773)(5108,1735)(5107,1698)
	(5107,1660)(5107,1622)(5107,1591)
	(5107,1559)(5108,1527)(5108,1494)
	(5109,1460)(5110,1424)(5111,1388)
	(5112,1350)(5113,1311)(5115,1270)
	(5117,1227)(5119,1182)(5121,1135)
	(5123,1086)(5126,1035)(5129,981)
	(5132,926)(5135,868)(5138,809)
	(5142,748)(5145,686)(5149,623)
	(5153,560)(5156,498)(5160,436)
	(5164,377)(5167,320)(5171,267)
	(5174,218)(5177,174)(5179,135)
	(5181,102)(5183,75)(5184,53)
	(5185,36)(5186,25)(5187,18)
	(5187,14)(5187,12)
\drawline(5637,2697)(5637,2695)(5636,2691)
	(5634,2684)(5631,2672)(5627,2656)
	(5621,2635)(5615,2609)(5607,2578)
	(5599,2543)(5590,2505)(5580,2464)
	(5570,2420)(5560,2376)(5550,2330)
	(5541,2285)(5531,2240)(5523,2196)
	(5514,2153)(5507,2111)(5500,2070)
	(5494,2031)(5489,1992)(5484,1954)
	(5480,1917)(5476,1881)(5473,1844)
	(5471,1808)(5469,1772)(5468,1735)
	(5467,1698)(5467,1659)(5467,1628)
	(5468,1597)(5468,1564)(5469,1531)
	(5471,1497)(5473,1461)(5475,1425)
	(5477,1386)(5480,1346)(5484,1305)
	(5488,1261)(5492,1215)(5496,1167)
	(5501,1117)(5507,1065)(5513,1010)
	(5519,953)(5526,894)(5533,833)
	(5541,770)(5548,706)(5556,642)
	(5564,577)(5572,513)(5580,450)
	(5588,388)(5595,330)(5602,275)
	(5609,225)(5615,179)(5620,139)
	(5625,105)(5628,77)(5631,54)
	(5634,37)(5635,25)(5636,18)
	(5637,14)(5637,12)
\drawline(6087,2712)(6086,2710)(6085,2706)
	(6083,2697)(6080,2684)(6075,2666)
	(6069,2642)(6061,2612)(6052,2577)
	(6042,2537)(6031,2492)(6019,2443)
	(6007,2392)(5994,2339)(5981,2284)
	(5969,2230)(5956,2175)(5945,2122)
	(5934,2069)(5923,2019)(5913,1970)
	(5904,1922)(5896,1877)(5889,1833)
	(5883,1791)(5877,1751)(5872,1711)
	(5868,1673)(5864,1636)(5862,1599)
	(5860,1563)(5858,1527)(5857,1491)
	(5857,1454)(5857,1422)(5858,1389)
	(5859,1356)(5861,1323)(5863,1288)
	(5866,1253)(5869,1217)(5873,1180)
	(5877,1141)(5882,1101)(5888,1059)
	(5894,1016)(5901,971)(5909,923)
	(5917,874)(5926,823)(5936,770)
	(5946,716)(5956,660)(5967,604)
	(5979,546)(5990,489)(6002,432)
	(6013,377)(6024,324)(6034,274)
	(6044,227)(6053,185)(6061,148)
	(6068,115)(6074,89)(6078,67)
	(6082,51)(6084,40)(6086,33)
	(6087,29)(6087,27)
\drawline(7422,2697)(7422,2695)(7423,2691)
	(7423,2683)(7425,2671)(7426,2654)
	(7429,2631)(7431,2602)(7435,2567)
	(7439,2526)(7443,2479)(7448,2428)
	(7454,2372)(7460,2312)(7466,2249)
	(7472,2185)(7478,2119)(7484,2053)
	(7490,1987)(7496,1922)(7501,1858)
	(7507,1796)(7512,1735)(7517,1677)
	(7521,1621)(7526,1568)(7530,1517)
	(7533,1468)(7536,1422)(7539,1377)
	(7542,1335)(7544,1295)(7546,1256)
	(7548,1219)(7549,1183)(7550,1148)
	(7551,1115)(7552,1082)(7552,1051)
	(7552,1019)(7552,979)(7551,939)
	(7550,900)(7549,862)(7547,824)
	(7544,786)(7541,747)(7537,708)
	(7533,668)(7528,628)(7523,586)
	(7517,543)(7510,498)(7503,453)
	(7496,407)(7488,360)(7480,314)
	(7472,268)(7464,224)(7456,183)
	(7448,145)(7442,111)(7436,82)
	(7431,58)(7428,40)(7425,27)
	(7423,19)(7422,14)(7422,12)
\drawline(7872,2697)(7872,2695)(7873,2691)
	(7874,2683)(7877,2671)(7880,2653)
	(7883,2630)(7888,2602)(7894,2567)
	(7901,2528)(7908,2484)(7916,2435)
	(7925,2383)(7933,2329)(7942,2273)
	(7951,2217)(7960,2160)(7968,2103)
	(7977,2048)(7985,1994)(7992,1941)
	(7999,1891)(8005,1842)(8011,1795)
	(8016,1750)(8021,1707)(8025,1666)
	(8029,1626)(8032,1587)(8035,1550)
	(8037,1513)(8039,1478)(8040,1443)
	(8041,1408)(8042,1374)(8042,1339)
	(8042,1305)(8041,1271)(8040,1237)
	(8039,1202)(8037,1166)(8035,1130)
	(8032,1094)(8029,1055)(8025,1016)
	(8021,975)(8016,933)(8011,889)
	(8005,843)(7999,796)(7992,746)
	(7985,695)(7977,643)(7968,589)
	(7960,534)(7951,478)(7942,423)
	(7933,369)(7925,316)(7916,266)
	(7908,219)(7901,176)(7894,138)
	(7888,104)(7883,77)(7880,54)
	(7877,37)(7874,25)(7873,18)
	(7872,14)(7872,12)
\drawline(6972,2697)(6972,2695)(6973,2691)
	(6975,2682)(6978,2669)(6982,2651)
	(6987,2626)(6993,2596)(7000,2559)
	(7009,2518)(7018,2471)(7029,2420)
	(7039,2366)(7051,2309)(7062,2251)
	(7073,2192)(7085,2133)(7096,2075)
	(7106,2018)(7116,1963)(7125,1910)
	(7134,1859)(7142,1810)(7149,1764)
	(7156,1721)(7162,1679)(7167,1640)
	(7171,1602)(7175,1567)(7178,1533)
	(7181,1501)(7183,1470)(7184,1440)
	(7185,1412)(7185,1384)(7185,1357)
	(7183,1321)(7181,1285)(7178,1250)
	(7174,1216)(7169,1182)(7164,1148)
	(7158,1115)(7151,1082)(7143,1050)
	(7135,1018)(7126,986)(7117,956)
	(7108,925)(7098,896)(7089,867)
	(7079,839)(7069,812)(7060,786)
	(7050,760)(7041,736)(7033,712)
	(7025,689)(7017,666)(7010,645)
	(7003,623)(6997,602)(6991,579)
	(6986,556)(6981,533)(6977,509)
	(6974,484)(6971,458)(6969,430)
	(6967,401)(6966,371)(6965,338)
	(6964,304)(6964,268)(6965,231)
	(6965,194)(6966,159)(6967,125)
	(6968,94)(6969,68)(6970,47)
	(6971,31)(6972,20)(6972,15)(6972,12)
\drawline(6522,2697)(6522,2695)(6521,2690)
	(6519,2681)(6517,2667)(6514,2648)
	(6510,2623)(6505,2591)(6499,2554)
	(6493,2511)(6485,2464)(6477,2414)
	(6469,2360)(6461,2305)(6452,2249)
	(6444,2193)(6436,2137)(6428,2083)
	(6420,2031)(6413,1980)(6407,1932)
	(6401,1887)(6395,1843)(6390,1802)
	(6385,1764)(6381,1727)(6378,1692)
	(6375,1660)(6372,1628)(6370,1598)
	(6368,1570)(6366,1542)(6365,1515)
	(6365,1489)(6364,1456)(6364,1424)
	(6364,1392)(6365,1361)(6367,1330)
	(6369,1299)(6371,1268)(6374,1238)
	(6377,1208)(6381,1178)(6385,1148)
	(6389,1119)(6393,1090)(6398,1061)
	(6403,1033)(6408,1006)(6413,979)
	(6418,952)(6423,926)(6428,901)
	(6433,876)(6437,852)(6442,828)
	(6446,804)(6450,781)(6455,757)
	(6458,733)(6462,709)(6466,684)
	(6469,658)(6472,630)(6476,602)
	(6479,571)(6482,539)(6485,505)
	(6489,468)(6492,429)(6495,388)
	(6499,346)(6502,302)(6505,258)
	(6508,215)(6511,173)(6514,135)
	(6516,100)(6518,72)(6520,49)
	(6521,32)(6521,21)(6522,15)(6522,12)
\drawline(8322,2262)(8320,2262)(8316,2262)
	(8308,2262)(8296,2263)(8279,2263)
	(8257,2264)(8230,2265)(8197,2266)
	(8159,2267)(8118,2269)(8073,2270)
	(8025,2271)(7975,2273)(7925,2274)
	(7874,2276)(7823,2277)(7773,2278)
	(7725,2279)(7677,2280)(7632,2281)
	(7587,2282)(7545,2282)(7504,2283)
	(7465,2283)(7427,2283)(7390,2283)
	(7354,2283)(7319,2283)(7284,2282)
	(7250,2282)(7215,2281)(7181,2280)
	(7147,2279)(7114,2278)(7082,2277)
	(7048,2276)(7014,2275)(6980,2273)
	(6945,2272)(6910,2270)(6874,2268)
	(6837,2267)(6800,2265)(6762,2263)
	(6724,2261)(6685,2258)(6646,2256)
	(6606,2254)(6567,2252)(6527,2250)
	(6487,2247)(6447,2245)(6407,2243)
	(6368,2241)(6329,2238)(6290,2236)
	(6252,2234)(6214,2232)(6177,2230)
	(6140,2229)(6104,2227)(6069,2225)
	(6034,2224)(6001,2222)(5967,2221)
	(5935,2220)(5902,2219)(5871,2218)
	(5840,2217)(5805,2216)(5770,2216)
	(5736,2215)(5701,2215)(5666,2215)
	(5631,2215)(5594,2215)(5557,2216)
	(5519,2216)(5479,2217)(5438,2218)
	(5395,2219)(5350,2221)(5304,2222)
	(5257,2224)(5208,2226)(5159,2228)
	(5109,2230)(5060,2232)(5012,2234)
	(4966,2237)(4924,2239)(4885,2240)
	(4851,2242)(4822,2243)(4798,2245)
	(4780,2246)(4767,2246)(4758,2247)
	(4754,2247)(4752,2247)
\drawline(8337,1804)(8335,1804)(8330,1804)
	(8321,1805)(8307,1806)(8288,1806)
	(8263,1808)(8232,1809)(8195,1811)
	(8154,1813)(8108,1815)(8059,1817)
	(8008,1819)(7956,1821)(7903,1823)
	(7851,1825)(7799,1826)(7749,1828)
	(7700,1829)(7653,1830)(7608,1831)
	(7564,1831)(7522,1831)(7482,1831)
	(7443,1831)(7405,1830)(7369,1829)
	(7332,1828)(7296,1827)(7261,1825)
	(7225,1823)(7190,1821)(7157,1818)
	(7125,1816)(7092,1813)(7059,1810)
	(7025,1807)(6991,1804)(6956,1800)
	(6921,1797)(6884,1793)(6848,1789)
	(6810,1785)(6772,1781)(6734,1776)
	(6695,1772)(6656,1767)(6617,1763)
	(6577,1759)(6538,1754)(6498,1750)
	(6459,1745)(6419,1741)(6380,1737)
	(6342,1733)(6303,1729)(6266,1725)
	(6229,1721)(6192,1718)(6156,1715)
	(6121,1712)(6086,1709)(6052,1707)
	(6018,1705)(5986,1703)(5953,1701)
	(5921,1699)(5890,1698)(5854,1697)
	(5819,1697)(5784,1696)(5749,1696)
	(5713,1697)(5677,1698)(5640,1699)
	(5601,1701)(5562,1703)(5521,1706)
	(5479,1709)(5434,1713)(5388,1717)
	(5341,1722)(5291,1727)(5241,1732)
	(5190,1738)(5138,1743)(5087,1749)
	(5038,1755)(4990,1761)(4946,1766)
	(4905,1771)(4870,1776)(4839,1780)
	(4815,1783)(4796,1785)(4782,1787)
	(4774,1788)(4769,1789)(4767,1789)
\drawline(8337,1354)(8335,1354)(8331,1354)
	(8323,1355)(8311,1355)(8294,1356)
	(8272,1357)(8244,1359)(8210,1360)
	(8171,1362)(8128,1364)(8081,1367)
	(8030,1369)(7977,1371)(7923,1374)
	(7868,1376)(7812,1378)(7758,1380)
	(7704,1382)(7652,1384)(7601,1385)
	(7553,1386)(7506,1387)(7461,1388)
	(7418,1389)(7377,1389)(7338,1389)
	(7301,1389)(7265,1389)(7230,1388)
	(7197,1387)(7164,1386)(7132,1384)
	(7101,1382)(7070,1380)(7040,1378)
	(7005,1375)(6972,1372)(6938,1369)
	(6903,1365)(6869,1361)(6835,1357)
	(6800,1352)(6765,1348)(6729,1343)
	(6693,1337)(6657,1332)(6620,1327)
	(6584,1321)(6547,1315)(6510,1310)
	(6473,1304)(6437,1298)(6400,1293)
	(6364,1288)(6328,1282)(6292,1277)
	(6257,1272)(6222,1268)(6187,1263)
	(6154,1259)(6120,1256)(6087,1252)
	(6055,1249)(6022,1247)(5991,1244)
	(5959,1242)(5927,1241)(5897,1240)
	(5867,1239)(5836,1238)(5805,1238)
	(5773,1239)(5741,1240)(5707,1241)
	(5672,1242)(5635,1244)(5597,1247)
	(5557,1250)(5515,1253)(5472,1257)
	(5426,1262)(5379,1266)(5330,1271)
	(5279,1277)(5228,1282)(5176,1288)
	(5124,1294)(5074,1300)(5025,1306)
	(4978,1312)(4935,1317)(4897,1322)
	(4863,1327)(4834,1330)(4811,1333)
	(4794,1335)(4781,1337)(4773,1338)
	(4769,1339)(4767,1339)
\drawline(8322,469)(8320,469)(8316,469)
	(8308,470)(8295,470)(8277,471)
	(8254,472)(8224,473)(8189,475)
	(8149,476)(8103,478)(8054,480)
	(8001,482)(7945,484)(7888,486)
	(7831,489)(7773,491)(7715,493)
	(7659,494)(7604,496)(7551,498)
	(7500,499)(7451,501)(7404,502)
	(7359,503)(7316,503)(7274,504)
	(7235,504)(7197,505)(7160,505)
	(7124,505)(7090,504)(7056,504)
	(7022,503)(6990,503)(6957,502)
	(6923,501)(6888,499)(6854,498)
	(6820,497)(6785,495)(6750,493)
	(6715,491)(6680,489)(6644,487)
	(6608,484)(6572,482)(6535,479)
	(6498,476)(6462,474)(6425,471)
	(6388,468)(6351,465)(6314,462)
	(6278,460)(6242,457)(6206,454)
	(6171,451)(6137,449)(6103,446)
	(6069,444)(6036,442)(6004,439)
	(5972,437)(5941,435)(5910,434)
	(5880,432)(5851,430)(5821,429)
	(5792,428)(5761,427)(5730,426)
	(5699,425)(5668,425)(5636,424)
	(5603,424)(5569,424)(5535,424)
	(5499,425)(5461,426)(5422,427)
	(5381,428)(5338,429)(5293,430)
	(5247,432)(5200,434)(5152,436)
	(5103,438)(5055,440)(5008,442)
	(4964,444)(4921,446)(4883,448)
	(4849,449)(4821,451)(4797,452)
	(4779,453)(4767,453)(4758,454)
	(4754,454)(4752,454)
\drawline(8322,906)(8320,906)(8316,906)
	(8309,907)(8297,908)(8280,909)
	(8258,910)(8230,912)(8197,914)
	(8159,916)(8116,919)(8069,922)
	(8019,925)(7967,928)(7913,931)
	(7858,934)(7804,937)(7749,940)
	(7696,943)(7644,946)(7593,948)
	(7545,950)(7498,952)(7453,954)
	(7410,955)(7368,957)(7328,958)
	(7290,959)(7253,959)(7217,960)
	(7183,960)(7149,960)(7115,959)
	(7082,959)(7050,958)(7017,957)
	(6983,956)(6948,955)(6914,954)
	(6879,952)(6844,950)(6808,948)
	(6772,946)(6736,943)(6699,941)
	(6662,938)(6624,935)(6586,932)
	(6548,929)(6509,926)(6471,922)
	(6432,919)(6394,916)(6356,912)
	(6317,909)(6280,906)(6242,902)
	(6205,899)(6169,896)(6133,893)
	(6098,890)(6063,887)(6029,884)
	(5996,882)(5963,879)(5931,877)
	(5899,875)(5868,873)(5837,871)
	(5807,869)(5775,868)(5743,867)
	(5711,866)(5678,865)(5645,864)
	(5612,864)(5577,864)(5542,864)
	(5505,864)(5467,864)(5427,865)
	(5385,866)(5342,867)(5297,868)
	(5250,870)(5203,871)(5154,873)
	(5105,875)(5057,877)(5010,879)
	(4964,881)(4922,883)(4884,885)
	(4850,886)(4821,888)(4798,889)
	(4780,890)(4767,890)(4758,891)
	(4754,891)(4752,891)
\dashline{60.000}(1812,1842)(1813,1842)(1817,1843)
	(1823,1844)(1833,1846)(1847,1849)
	(1867,1853)(1892,1858)(1922,1865)
	(1958,1872)(2000,1880)(2048,1890)
	(2101,1900)(2159,1912)(2222,1924)
	(2289,1937)(2359,1951)(2431,1965)
	(2506,1979)(2582,1994)(2659,2008)
	(2736,2022)(2813,2036)(2889,2050)
	(2965,2063)(3038,2076)(3111,2088)
	(3181,2100)(3249,2111)(3316,2121)
	(3380,2131)(3443,2140)(3503,2148)
	(3561,2156)(3617,2163)(3672,2170)
	(3725,2175)(3776,2180)(3826,2185)
	(3875,2189)(3923,2192)(3969,2195)
	(4015,2197)(4060,2198)(4104,2199)
	(4148,2200)(4191,2200)(4235,2199)
	(4279,2198)(4324,2197)(4369,2195)
	(4414,2192)(4459,2189)(4504,2185)
	(4549,2180)(4596,2175)(4643,2169)
	(4691,2163)(4739,2155)(4790,2147)
	(4841,2138)(4894,2129)(4948,2118)
	(5004,2107)(5061,2095)(5120,2082)
	(5180,2069)(5243,2054)(5306,2039)
	(5371,2024)(5437,2008)(5503,1991)
	(5571,1974)(5638,1956)(5704,1939)
	(5770,1922)(5834,1904)(5896,1888)
	(5955,1871)(6012,1856)(6064,1842)
	(6112,1828)(6155,1816)(6193,1805)
	(6226,1796)(6254,1788)(6277,1782)
	(6294,1776)(6308,1773)(6327,1767)
\blacken\drawline(6203.536,1774.528)(6327.000,1767.000)(6221.604,1831.743)(6203.536,1774.528)
\dashline{60.000}(1302,1377)(1303,1377)(1307,1378)
	(1313,1379)(1323,1381)(1337,1384)
	(1357,1388)(1382,1393)(1412,1400)
	(1448,1407)(1490,1415)(1538,1425)
	(1591,1435)(1649,1447)(1712,1459)
	(1779,1472)(1849,1486)(1921,1500)
	(1996,1514)(2072,1529)(2149,1543)
	(2226,1557)(2303,1571)(2379,1585)
	(2455,1598)(2528,1611)(2601,1623)
	(2671,1635)(2739,1646)(2806,1656)
	(2870,1666)(2933,1675)(2993,1683)
	(3051,1691)(3107,1698)(3162,1705)
	(3215,1710)(3266,1715)(3316,1720)
	(3365,1724)(3413,1727)(3459,1730)
	(3505,1732)(3550,1733)(3594,1734)
	(3638,1735)(3681,1735)(3725,1734)
	(3769,1733)(3814,1732)(3859,1730)
	(3904,1727)(3949,1724)(3994,1720)
	(4039,1715)(4086,1710)(4133,1704)
	(4181,1698)(4229,1690)(4280,1682)
	(4331,1673)(4384,1664)(4438,1653)
	(4494,1642)(4551,1630)(4610,1617)
	(4670,1604)(4733,1589)(4796,1574)
	(4861,1559)(4927,1543)(4993,1526)
	(5061,1509)(5128,1491)(5194,1474)
	(5260,1457)(5324,1439)(5386,1423)
	(5445,1406)(5502,1391)(5554,1377)
	(5602,1363)(5645,1351)(5683,1340)
	(5716,1331)(5744,1323)(5767,1317)
	(5784,1311)(5798,1308)(5817,1302)
\blacken\drawline(5693.536,1309.528)(5817.000,1302.000)(5711.604,1366.743)(5693.536,1309.528)
\put(1497,1152){\makebox(0,0)[lb]{\smash{{\SetFigFontNFSS{12}{14.4}{\rmdefault}{\mddefault}{\updefault}$X$}}}}
\put(6042,1347){\makebox(0,0)[lb]{\smash{{\SetFigFontNFSS{12}{14.4}{\rmdefault}{\mddefault}{\updefault}$Y$}}}}
\put(4077,1917){\makebox(0,0)[lb]{\smash{{\SetFigFontNFSS{12}{14.4}{\rmdefault}{\mddefault}{\updefault}$\phi$}}}}
\end{picture}
}

